Temporal Graph Rewiring with Expander Graphs

Evolving relations in real-world networks are often modelled by temporal graphs. Temporal Graph Neural Networks (TGNNs) emerged to model evolutionary behaviour of such graphs by leveraging the message passing primitive at the core of Graph Neural Networks (GNNs). It is well-known that GNNs are vulnerable to several issues directly related to the input graph topology, such as under-reaching and over-squashing - we argue that these issues can often get exacerbated in temporal graphs, particularly as the result of stale nodes and edges. While graph rewiring techniques have seen frequent usage in GNNs to make the graph topology more favourable for message passing, they have not seen any mainstream usage on TGNNs. In this work, we propose Temporal Graph Rewiring (TGR), the first approach for graph rewiring on temporal graphs, to the best of our knowledge. TGR constructs message passing highways between temporally distant nodes in a continuous-time dynamic graph by utilizing expander graph propagation, a prominent framework used for graph rewiring on static graphs which makes minimal assumptions on the underlying graph structure. On the challenging TGB benchmark, TGR achieves state-of-the-art results on tgbl-review, tgbl-coin, tgbl-comment and tgbl-flight datasets at the time of writing. For tgbl-review, TGR has 50.5% improvement in MRR over the base TGN model and 22.2% improvement over the base TNCN model. The significant improvement over base models demonstrates clear benefits of temporal graph rewiring.

==> A2EGP.tex <==
\section{Expander Graph Propagation}
\label{section:003.4}
Expander Graph Propagation (EGP) framework is simplistic in nature and shows incredibly favourable properties for rewiring on static graphs: relieving information bottleneck and oversquashing, while maintaining low computational cost and subquadratic time. For a set of input node features $\mathbf{X}^{n \times d}$, where $n$ is the number of nodes and $d$ is the feature vector size, EGP operates by alternating GNN layers and propagating them over the adjacency matrix of the input graph and Cayley graph in a following manner:

\begin{equation}
    \mathbf{H} = \text{GNN}(\text{GNN}(\mathbf{X}, \mathbf{A}), \mathbf{A}^{Cay}).
\end{equation}

Here, $\mathbf{H}$ represents node embedding vector generated after EGP forward pass, and $\mathbf{A}$ and $\mathbf{A}^{Cay}$ are the adjacency matrices for the input and Cayley graph respectively. A $\text{GNN}$ can be any classical GNN layer, such as graph attentional network (GAT) \cite{velivckovic2017graph}:

\begin{equation}
    \mathbf{h}_i = \underset{k=1}{\overset{K}{{\bigg\|}}} \sigma \left( \sum_{j \in \mathcal{N}_i} \alpha_{ij}^k \mathbf{W}^k \mathbf{x}_j \right).
\end{equation}
In the equation above for multi-head-attention layer, $i$ is a node of interest and $\mathcal{N}_i$ is its direct neighbourhood, $\alpha_{ij}^k$ are the attention weights of the $k$-th attention head and $\mathbf{W}^k$ is corresponding input linear transformation's weight matrix.

==> hyperparameters2.tex <==
\begin{table}[h]
\centering
\caption{Parameter settings for different datasets.}
\begin{tabular}{lccc}
\toprule
Dataset & num\_neighbors & num\_epoch & patience \\
\midrule
Wiki     & 10 & 20 & 5 \\
Review   & 10 & 5  & 2 \\
Coin     & 10 & 3  & 2 \\
Comment  & 10 & 3  & 1 \\
\bottomrule
\end{tabular}
\end{table}

==> lowhightable1.tex <==
% Define the color for highlighting
\definecolor{lightgreen}{rgb}{0.56, 0.93, 0.56}

\begin{table}[h]
\caption{Test MRR depending on choice of expander nodes highlighting our choice of mixing level parameter. \textbf{"b"} denotes \textit{batch} mode and \textbf{"b+n"} denotes \textit{batch and 1-hop neighbours} mode.
}
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & {\texttt{tgbl-wiki}} & {\texttt{tgbl-review}} & {\texttt{tgbl-coin}} & {\texttt{tgbl-comment}} & {\texttt{tgbl-flight}} \\
\midrule
TGR-TGN (b+n)  & 32.3 & \textbf{85.4} & 60.9 & 63.1 & \textbf{76.2} \\
TGR-TGN (b)   & \textbf{58.9} & 79.6               & \textbf{75.4}  & \textbf{72.9}                & 70.9                \\
\midrule
TGR-TNCN (b+n)        & 22.4               & \textbf{59.9}          & 33.9          & 49.9           & 54.9          \\
TGR-TNCN (b)  & \textbf{72.4} & 46.6          & 
\textbf{78.3} & \textbf{89.1} & \textbf{85.1}\\
\bottomrule
\end{tabular}
\label{as1}
\end{table}
